Automated Tour Design in the Saturnian System

Future missions to Enceladus would benefit from multi-moon tours that leverage V-infinity on resonant orbits to progressively transfer between moons. Such "resonance family hopping" trajectories present a vast search space for global optimization due to the different combinations of available resonances and flyby speeds. The proposed multi-objective tour design algorithm optimizes entire moon tours from Titan to Enceladus via grid-based dynamic programming, in which the computation time is significantly reduced by utilizing a database of V-infinity-leveraging transfers. The result unveils a complete trade space of the moon tour design to Enceladus in a tractable computation time and global optimality.

==> Tables/f_to_theta.tex <==
\begin{table} 
\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{c c c} 
 \hline
$(p,q)$ & $\theta_1 (^{\circ})$ & $\theta_2 (^{\circ})$ \\ 
 \hline\hline
$(1,1)$ & $180 - |f| + 360 a$ & $180 + |f| + 360b$  \\ 
$(-1,-1)$ & $180 + |f| +360 a$ & $180 - |f| + 360b$  \\ 
$(1,-1)$ & $180 - |f| + 360 a$ & $180 - |f| + 360b$  \\
$(-1,1)$ & $180 + |f| + 360 a$ & $180 + |f| + 360 b$  \\  
 \hline
\end{tabular}
\caption{ $M > N$ (Exterior transfer)}
\label{tab:table1_a}
\end{subtable} 

\begin{subtable}[t]{\textwidth}\centering
\begin{tabular}{l c c} 
 \hline
 & $\theta_1 (^{\circ})$ & $\theta_2 (^{\circ})$ \\ 
 \hline\hline
$(p,q) = (1,1)$   & $360 - |f| + 360 a$ & $|f| + 360 b$ \\ 
$(p,q) = (-1,-1)$ & $|f| + 360 a $      & $|f| + 360 b$ \\ 
$(p,q) = (1,-1)$  & $360 - |f| + 360 a$ & $360 - |f| + 360 b$  \\
$(p,q) = (-1,1)$  & $|f| + 360 a$       & $360 - |f| + 360 b$  \\  
 \hline
\end{tabular}
\caption{ $M < N$ (Interior transfer)}
\label{tab:table1_a}
\end{subtable}

\begin{subtable}[t]{\textwidth} \centering
\begin{tabular}{l c c}
 \hline
 & $\theta_1 (^{\circ})$ & $\theta_2 (^{\circ})$ \\ 
 \hline\hline
$(p,q) = (1,1)$   & $360 - |f|$ & $|f|$  \\ 
$(p,q) = (-1,-1)$ & $|f|$       & $360 - |f|$  \\ 
$(p,q) = (1,-1)$  & $360 - |f|$ & $360 - |f|$  \\
$(p,q) = (-1,1)$  & $|f| + 180$ & $|f| + 180$  \\  
 \hline
\end{tabular}
\caption{ $M = N = 1$}
\label{tab:table1_a}
\end{subtable}

\caption{Conversion from $|f|$ to $\theta_1$ and $\theta_2$. $a=\text{floor}((N-1)/2)$ and $b=N-1-a$.}
\label{tab:f_to_theta}
\end{table}

==> Tables/f_to_theta2.tex <==
\begin{table}[h!]
\fontsize{9}{9}\selectfont
\centering
\begin{tabular}{c|c c|c c|c c} 
\hline
 & \multicolumn{2}{c}{Exterior $(M>N)$} & \multicolumn{2}{c}{Interior $(M<N)$} & \multicolumn{2}{c}{$M=N=1$}\\
$(p,q)$ & $\theta_1$ (rad) & $\theta_2$ (rad) & $\theta_1$ (rad) & $\theta_2$ (rad) & $\theta_1$ (rad) & $\theta_2$ (rad) \\ 
\hline\hline
$(1,1)$ & $2\pi (a+\frac{1}{2}) - |f|$ & $2\pi(b+\frac{1}{2})+|f|$ &  $2\pi(a+1) - |f|$ & $2\pi b+|f|$ & $2\pi - |f|$ & $|f|$  \\
$(-1,-1)$ & $2\pi (a+\frac{1}{2}) + |f|$ & $2\pi(b+\frac{1}{2})-|f|$ & $2\pi a + |f|$ & $2\pi (b+1) - |f|$ & $|f|$ & $2\pi - |f|$  \\
$(1,-1)$ & $2\pi (a+\frac{1}{2}) - |f|$ & $2\pi(b+\frac{1}{2})-|f|$ & $2\pi(a+1) - |f|$ & $2\pi (b+1) - |f|$ & $2\pi - |f|$ & $2\pi - |f|$\\
$(-1,1)$ & $2\pi (a+\frac{1}{2}) + |f|$ & $2\pi(b+\frac{1}{2})+|f|$ & $2\pi a + |f|$ & $2\pi b+|f|$ & $\pi+|f|$ & $\pi+|f|$  \\
\hline
\end{tabular}
\caption{Conversion from $f$ to $\theta_1$ and $\theta_2$. $a=\text{floor}((N-1)/2)$ and $b=N-1-a$.}
\label{tab:sum_tour}
\end{table}

==> Tables/nomenclature.tex <==
\subsection{Variables}

\begin{tabular}[h!]{r l}
    $a$ & semimajor axis \\
    $e$ & eccentricity \\
    $GM$ & gravitational parameter \\
    $h$ & angular momentum \\
    $i$ & inclination \\ 
	$M$ & Moon revolution \\
	$N$ & Spacecraft revolution \\
	$p$ & inbound/outbound at departure \\
	$q$ & inbound/outbound at arrival \\
    $\textbf{r}$ & position vector of spacecraft \\
	$r_a$ & apoapsis radius \\
	$r_M$ & radius of Moon \\
	$\textbf{r}_M$ & position vector of Moon \\
	$r_p$ & periapsis radius \\
	$V_\infty$ & excess velocity \\
	$\alpha$ & pump angle \\
	$\Delta V$ & change in velocity \\
    $\theta$ & transfer angle (in true anomaly) 
\end{tabular} \\

\subsection{Subscripts / Superscripts}

\begin{tabular}[h!]{r l}
    $x_{arr}$ & `x' is quantity at arrival of the resonance \\
	$x_{dep}$ & `x' is quantity at departure of the resonance  \\
	$x_{M}$ & `x' is quantity of Moon  \\
	$x_{S}$ & `x' is quantity of Saturn  \\
	$x_{SC}$ & `x' is quantity of spacecraft  \\
    $x^{k}$ & `x' is quantity at $k$-th flyby 
\end{tabular} \\


